Temporal complex networks modeling applied to vehicular ad-hoc networks

VANETs solutions use aggregated graph representation to model the interaction among the vehicles and different aggregated complex network measures to quantify some topological characteristics. This modeling ignores the temporal interactions between the cars, causing loss of information or unrealistic behavior. This work proposes the use of both temporal graphs and temporal measures to model VANETs applications. To verify the viability of this model, we initially perform a comparative analysis between the temporal and aggregated modeling considering five different real datasets. This analysis shows that the aggregated model is inefficient in modeling the temporal aspects of networks. After that, we perform a network evaluation through a simulation by considering the impact of temporal modeling applied to the deployment of RSUs. First, we compare a solution based on our temporal modeling with a greedy algorithm based on an aggregated model to choose the positions of RSUs. In a scenario with 70 RSUs, we have 77% and 65% of coverage in the temporal and aggregated model (greedy algorithm), respectively. Second, we evaluate the use of aggregated and temporal measures applied as features in a genetic algorithm. The approach with temporal betweenness had the better result with 90% of the coverage area against 61% of aggregated one applied to the same scenario.

==> grafos/contact_matrix.tex <==
\begin{figure}[!htb]
\centering
    \begin{subfigure}[t]{0.4\textwidth}
		% $\mathcal{T}_{\textbf{G}}$ = 
        \begin{tabular}{@{}c|cccccc@{}}
              & $v_1$ & $v_2$ & $v_3$ & $v_4$ & $v_5$ \\ \midrule
        $I_1$ & 1 & 1 & 1 & 0 & 1 \\ 
        $I_2$ & 0 & 1 & 1 & 1 & 0 \\ 
        \end{tabular}
        \caption{$\mathcal{T}_{G}$}
        	\label{fig:contact_matrix_a}
    \end{subfigure}
	\begin{subfigure}[t]{0.4\textwidth}
        \begin{tabular}{@{}c|cccccc@{}}
            & $v_1$ & $v_2$ & $v_3$ & $v_4$ & $v_5$ \\ \midrule
        $I_1$ & 2 & 1 & 1 & 0 & 2 \\ 
        $I_2$ & 0 & 2 & 2 & 3 & 0 \\ 
        \end{tabular}
        \caption{$\mathcal{T}^{[1,3]}_{\mathcal{G}}$}
        	\label{fig:contact_matrix_t}
    \end{subfigure}
    	\caption{Contact matrix to the aggregated and the temporal graph.}
    	\label{fig:contact_matrix}
\end{figure}

\begin{figure}[!htb]
    %Time 1
    \centering
	\begin{subfigure}[b]{0.12\textwidth}
    	\centering
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.8cm,thick,
        main node/.style={circle,fill=black!0,draw,minimum size=0.4cm,inner sep=0pt, line width=1pt},
        font=\sffamily\scriptsize,
        main edge/.style={line width=1pt,dashed}
        ]
        
        \node[main node,fill=black!10] (I1) {$\textbf{I1}$};
        \node[main node,left of=I1] (A) {$v_1$};
        \node[main node] (B) [right of=I1]  {$v_2$};
        \node[main node] (E) [below left of=A] {$v_5$};
        \node[main node,fill=black!10,below of=I1] (I2) {$\textbf{I2}$};
        \node[main node] (C) [below left of=I2] {$v_3$};
        \node[main node] (D) [below right of=I2]  {$v_4$};
        \path[-]
        (A) edge[main edge] node {} (I1)
        (B) edge[main edge] node {} (I1)
        (C) edge[main edge] node {} (I2)
        (D) edge[main edge] node {} (I2);
        \end{tikzpicture}
        \caption*{\textbf{$t=1$}}
	\end{subfigure}%
	\hspace{2cm}
    %Time 2    
    \begin{subfigure}[b]{0.12\textwidth}
    	\centering
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.8cm,thick,
        main node/.style={circle,fill=black!0,draw,minimum size=0.4cm,inner sep=0pt, line width=1pt},
        font=\sffamily\scriptsize,
        main edge/.style={line width=1pt,dashed}
        ]
        
        \node[main node,fill=black!10] (I1) {$\textbf{I1}$};
        \node[main node,above left of=I1] (A) {$v_1$};
        \node[main node] (B) [below left of=I2]  {$v_2$};
        \node[main node] (E) [right of=I1] {$v_5$};
        
        \node[main node,fill=black!10,below of=I1] (I2) {$\textbf{I2}$};
        \node[main node] (B) [below left of=I2]  {$v_2$};
        \node[main node] (C) [right of=I2] {$v_3$};
        \node[main node] (D) [below right of=I2]  {$v_4$};
        \path[-]
        (E) edge[main edge] node {} (I1)
        (A) edge[main edge] node {} (I1)
        (C) edge[main edge] node {} (I2)
        (B) edge[main edge] node {} (I2)
        (D) edge[main edge] node {} (I2);
        \end{tikzpicture}
%          \begin{tikzpicture}
% 	  		\draw[-|,shorten <= -0.4cm,shorten >= -0.8cm, line width=0.3mm, black] node[below] {} ++(-2,0) -- node[above] {} ++(1.6,0);
% 		\end{tikzpicture}
%         \vspace{-2em}
        \caption*{\textbf{$t=2$}}
	\end{subfigure}%
	\hspace{1cm}
%      %Time 3
	\begin{subfigure}[b]{0.12\textwidth}
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=0.8cm,thick,
        main node/.style={circle,fill=black!0,draw,minimum size=0.4cm,inner sep=0pt, line width=1pt},
        font=\sffamily\scriptsize,
        main edge/.style={line width=1pt,dashed}
        ]
        \node[main node,fill=black!10] (I1) {$\textbf{I1}$};
        \node[main node] (E) [above right of=I1] {$v_5$};
        \node[main node] (C) [left of=I1] {$v_3$};
        \node[main node,below left of=C] (A) {$v_1$};
        \node[main node,fill=black!10,below of=I1] (I2) {$\textbf{I2}$};
        \node[main node] (B) [right of=I2]  {$v_2$};
        \node[main node] (D) [below right of=I2]  {$v_4$};
        \path[-]
        
        (C) edge[main edge] node {} (I1)
        (E) edge[main edge] node {} (I1)
        (D) edge[main edge] node {} (I2)
        (B) edge[main edge] node {} (I2);
        
        \end{tikzpicture}
%          \begin{tikzpicture}
% 	  		\draw[->,shorten <= -0.8cm,shorten >= -0.4cm, line width=0.3mm, black] node[below] {} ++(0,0) -- node[above] {} ++(2.5,0);
% 		\end{tikzpicture}
% 		\vspace{-2em}
        \caption*{$t=3$}
	\end{subfigure}
	\caption{Vehicles and intersections interactions in the time interval $[1, 3]$.}
	\label{fig:graph_contact_matrix}
\end{figure}




